A packet-level digital hardware twin for commissioning megahertz diagnostic edge AI and plasma control system integration in tokamaks

High-bandwidth plasma diagnostics increasingly provide inputs to machine learning and signal-processing algorithms intended for real-time tokamak control, but the complete path from diagnostic sampling to control-system handoff is difficult to commission because of their sampling rates. We develop a packet-level digital hardware twin for the megahertz diagnostic edge-AI architecture. The simulator represents a 64-channel, 1 MHz beam emission spectroscopy (BES) diagnostic embedded in a 96-channel dual-carrier acquisition system, two 48-channel streams with SPAD0 sample counters, 10 GbE Hardware UDP transport, packet loss and network jitter, FPGA parsing and dual-carrier alignment, causal preprocessing and edge inference, a compact Ethernet result packet, receiver-side shared state, and a 1 kHz PCS-like control cycle. Binary UDP payloads and PCAP files are generated rather than emulating transport only at the array level. With a baseline of 20 samples per packet, each carrier generates 50,000 packets s$^{-1}$ and 100 MB s$^{-1}$ of user payload. A 110 ms reference run produces 11,000 HUDP packets; an intentionally dropped 20-sample packet is detected by the sample-counter continuity logic and invalidates the two overlapping 128-sample inference windows without silent interpolation. For valid windows, the configured engineering latency model gives a median last-input-to-shared-memory latency of 91.6 us and a 99th percentile of 108.1 us. A separate operating-system loopback test sends binary FPGA-result datagrams through a UDP receiver into POSIX shared memory and preserves packet sequence and CRC for 20/20 packets. Interactive GUI interfaces expose timing, packetization, network faults, inference thresholds, and control-state inspection. The framework provides a reproducible environment for testing diagnostic-to-accelerator interfaces and fail-safe behavior for deployment on fusion devices.

==> my_macro.tex <==
\usepackage{color}

%% BRACKETS
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lab}{\left<}
\newcommand{\rab}{\right>}
\newcommand{\lsb}{\left[}
\newcommand{\rsb}{\right]}
\newcommand{\lcb}{\left\{}
\newcommand{\rcb}{\right\}}
\newcommand{\labs}{\left|}
\newcommand{\rabs}{\right|}

%%Referencing
\newcommand{\refeq}[1]{Equation (\ref{#1})}
\newcommand{\refsec}[1]{Section \ref{#1}}
\newcommand{\refapp}[1]{Appendix \ref{#1}}
\newcommand{\reffig}[1]{Figure \ref{#1}}
\newcommand{\refmultifig}[2]{Figures \ref{#1} and \ref{#2}}
\newcommand{\reftable}[1]{Table \ref{#1}}

%%Comments & Correction
\newcommand{\correction}[1]{\textcolor{black}{#1}}
\newcommand{\comment}[1]{\textcolor{blue}{#1}}

%%MATH NOTATION
\newcommand{\abs}[1]{\labs #1 \rabs}
\newcommand{\grad}{\nabla}
\newcommand{\tor}{\Phi}

%% INSTITUTIONS
\newcommand{\KAISTNQe}{Department of Nuclear and Quantum Engineering, KAIST, Daejeon 34141, Republic of Korea}
\newcommand{\JET}{EUROfusion Consortium JET Culham Science Centre, Abingdon OX14 3DB, United Kingdom}
\newcommand{\MaxPlanckGreifswald}{Max-Planck-Institut f$\ddot{u}$r Plasmaphysik, Teilinstitut Greifswald, D-17491 Greifswald, Germany}
\newcommand{\CCFE}{Culham Centre for Fusion Energy, Culham Science Centre, Abingdon OX14 3DB, United Kingdom}
\newcommand{\KFE}{Korea Institute of Fusion Energy, Daejeon 34133, Republic of Korea}
\newcommand{\Wigner}{Wigner RCP, Euratom Association-HAS, Budapest, Hungary}
\newcommand{\culham}{EURATOM/CCFE Fusion Association, Culham Science Centre, Abingdon, OX14 3DB, UK}
\newcommand{\MOBIIS}{Mobiis Co., Ltd., Seongnam-si, Gyeonggi-do 13486, Republic of Korea}
\newcommand{\UWMadison}{Department of Engineering Physics, University of Wisconsin-Madison, Madison, WI 53706, USA}
\newcommand{\PU}{Department of Mechanical and Aerospace Engineering, Princeton University, Princeton, NJ 08544,
USA}
\newcommand{\GA}{General Atomics, San Diego, CA 85608, USA}
\newcommand{\SLAC}{SLAC National Accelerator Lab, Menlo Park, CA 94025, USA}
\newcommand{\ANL}{Argonne National Laboratory, Lemont, IL 60439, USA}
\newcommand{\CU}{Columbia University, New York, NY 10027, USA}
\newcommand{\PPPL}{Princeton Plasma Physics Laboratory, Princeton, NJ 08540, USA}
\newcommand{\UCLA}{Department of Physics and Astronomy, University of California Los Angeles, Los Angeles, CA 90095, USA}

%% PEOPLE
\newcommand{\smjoung}{\author{Semin~Joung}\email[]{semin.joung@wisc.edu}\affiliation{\UWMadison}}
\newcommand{\jwkim}{\author{Jaewook~Kim}\affiliation{\KFE}}
\newcommand{\arfield}{\author{A.~R.~Field}\affiliation{\culham}}
\newcommand{\yunam}{\author{Y.U.~Nam}\affiliation{\KFE}}
\newcommand{\mlampert}{\author{M.~Lampert}\affiliation{\Wigner}}
\newcommand{\szoletnik}{\author{S.~Zoletnik}\affiliation{\Wigner}}
\newcommand{\ycghim}{\author{Y.-c.~Ghim}\affiliation{\KAISTNQe}}
\newcommand{\shkwak}{\author{Sehyun~Kwak}\affiliation{\KAISTNQe}\affiliation{\MaxPlanckGreifswald}}
\newcommand{\jsvensson}{\author{J.~Svensson}\affiliation{\MaxPlanckGreifswald}}
\newcommand{\mbrix}{\author{M.~Brix}\affiliation{\CCFE}}
\newcommand{\jetcontributor}{\author{JET Contributors}\email[]{See the Appendix of F. Romanelli et al., Proceedings of the 25th IAEA Fusion Energy Conference 2014, Saint Petersburg, Russia}\affiliation{\JET}}
\newcommand{\ymjeon}{\author{Y.M.~Jeon}\affiliation{\KFE}}
\newcommand{\shhahn}{\author{S.H.~Hahn}\affiliation{\KFE}}
\newcommand{\hshan}{\author{H.S.~Han}\affiliation{\KFE}}
\newcommand{\hskim}{\author{H.S.~Kim}\affiliation{\KFE}}
\newcommand{\jgbak}{\author{J.G.~Bak}\affiliation{\KFE}}
\newcommand{\sglee}{\author{S.G.~Lee}\affiliation{\KFE}}
\newcommand{\ghlee}{\author{Geunho~Lee}\affiliation{\MOBIIS}}
\newcommand{\dhkwon}{\author{Daeho~Kwon}\affiliation{\KAISTNQe}\affiliation{\MOBIIS}}
\newcommand{\drsmith}{\author{D.~R.~Smith}\email[]{david.smith@wisc.edu}\affiliation{\UWMadison}}
\newcommand{\gmckee}{\author{G.~McKee}\affiliation{\UWMadison}}
\newcommand{\fkhabanov}{\author{F.~Khabanov}\affiliation{\UWMadison}}
\newcommand{\kgill}{\author{K.~Gill}\affiliation{\UWMadison}}
\newcommand{\zyan}{\author{Z.~Yan}\affiliation{\UWMadison}}
\newcommand{\bgeiger}{\author{B.~Geiger}\affiliation{\UWMadison}}
\newcommand{\jzim}{\author{J.~Zimmerman}\affiliation{\UWMadison}}
\newcommand{\rcoffee}{\author{R.~Coffee}\affiliation{\SLAC}}
\newcommand{\lscomparin}{\author{L.~Scomparin}\affiliation{\SLAC}}
\newcommand{\adave}{\author{A.~Dave}\affiliation{\SLAC}}
\newcommand{\foshea}{\author{F.~H.~O'Shea}\affiliation{\SLAC}}
\newcommand{\ajalalvand}{\author{A.~Jalalvand}\affiliation{\PU}}
\newcommand{\ekolemen}{\author{E.~Kolemen}\affiliation{\PU}}
\newcommand{\asamaddar}{\author{A.~Samaddar}\affiliation{\ANL}}
\newcommand{\smadireddy}{\author{S.~Madireddy}\affiliation{\ANL}}
\newcommand{\chansen}{\author{C.~Hansen}\affiliation{\CU}}
\newcommand{\febrahimi}{\author{F.~Ebrahimi}\email[]{ebrahimi@pppl.gov}\affiliation{\PPPL}}
\newcommand{\sku}{\author{S.~Ku}\affiliation{\PPPL}}
\newcommand{\lschmitz}{\author{L.~Schmitz}\affiliation{\UCLA}}
\newcommand{\sdstewart}{\author{S.~D.~Stewart}\affiliation{\UWMadison}}
